Static Application Security Testing of Consensus-Critical Code in the Cosmos Network

Blockchains require deterministic execution in order to reach consensus. This is often guaranteed in languages designed to write smart contracts, such as Solidity. Application-specific blockchains or ``appchains'' allow the blockchain application logic to be written using general-purpose programming languages, giving developers more flexibility but also additional responsibilities. In particular, developers must ensure that their blockchain application logic does not contain any sources of non-determinism. Any source of non-determinism may be a potential source of vulnerabilities. This paper focuses on the use of Static Application Security Testing (SAST) tools to detect such sources of non-determinism at development time. We focus on Cosmos, a prominent open-source project that lets developers build interconnected networks of application-specific blockchains. Cosmos provides a Software Development Kit (SDK) that allows these chains to be implemented in the Go programming language. We create a corpus of 11 representative Cosmos-based appchains to analyze for sources of non-determinism in Go. As part of our study, we identified cosmos-sdk-codeql, a set of CodeQL code analysis rules for Cosmos applications. We find that these rules generate many false positives and propose a refactored set of rules that more precisely detects sources of non-determinism only in code that runs as part of the blockchain logic. We demonstrate a significant increase in the precision of the rules, making the SAST tool more effective and hence potentially contributing to enhanced security for Cosmos-based blockchains.

==> Assets/tables/uesless-3-3-overview-of-chains.tex <==
{\renewcommand{\arraystretch}{1.4}
    \begin{table*}[htp]
    \centering
    \caption{Vulnerabilities in Cosmos-based blockchains.}
    \label{tab:rules}
    \begin{tabularx}{\linewidth}{lX}
        \toprule
        \textbf{Vulnerability ID and name} & \textbf{Explanation} \\\midrule
        1. \{Begin,End\}Block panic & Panics in \texttt{\{Begin,End\}Block} ABCI calls will halt the chain and should never occur \cite{notsosmart} \cite{gosec-issues}. \\
         2. Map iteration & Iterating over a map in Go is non-deterministic and should be avoided when possible. If needed, an iteration over an array of the sorted keys should be used instead \cite{notsosmart} \cite{gosec-issues} \cite{maprange-vuln1}. \\
         3. Hardcoded Bech32 prefix & Bech32 prefixes should not be hardcoded because other modules might use the wrong address values. Instead, they should be configured using the Cosmos SDK's API \cite{gosec-issues} \cite{bech32-vuln1} \cite{bech32-vuln2}. \\
         4. Goroutines & Concurrency using goroutines and select statements are non-deterministic and should be avoided \cite{notsosmart} \cite{gosec-issues}. \\
         5. Floating point arithmetic & Floating point arithmetic can lead to unexpected results and should be avoided when possible. If needed, the operations should be converted into a form that can not result in unexpected behavior \cite{notsosmart} \cite{floating-incident}.\\
        6. System time & System clock times are not synchronized over the network and should never be used to validate or change state \cite{systemtime-vulnerability} \cite{provenance-chain}. \\
        7. Unsafe packages & Some packages contain functions that have unexpected results and are nondeterministic. Such packages include \textit{rand}, \textit{reflect}, \textit{unsafe} and \textit{runtime}, and should be avoided \cite{notsosmart} \cite{gosec-issues}. \\
        8. Platform-dependent types & Using platform-dependent types (e.g. \texttt{int}) can have different results on different architectures and should be avoided \cite{notsosmart}. \\ 
        \bottomrule
    \end{tabularx}
    \vspace{2cm}
    \caption{The corpus of the 11 blockchains used in this paper to analyze queries and vulnerabilities. \textit{Date} is the release of the first version. \textit{Total Tx} is the amount of transactions over a span of 7 days, between 25 May 2023 and 31 May 2023. \textit{\#Func} is the total amount of consensus-critical functions.}
        \label{tab:chains}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Name} & \textbf{Use case} & \textbf{Date} & \textbf{Total Tx} & \textbf{\# Func}\\\midrule
            Stride & A liquid staking platform. & 4 Sept. 2022 & 546,690 & 209\\
            Osmosis & The largest interchain decentralized exchange. & 16 June 2021 & 607,470 & 1310\\
            Gaia & The economic center of Cosmos providing IBC security and more. & 13 Aug. 2019 & 289,710 & 6 \\
            Axelar & Web3 integration across multiple chains & 8 Mar. 2021 & 2,944,100 & 2965\\
            Crypto.org & Payment, DeFi and NFTs. & 14 Oct. 2020 & 167,040 & 92\\
            Fetch.ai & Automation of Web3 systems using AI agents. & 1 July 2020 & 264,000 & 2\\
            Regen & Originate and invest in ecological regeneration projects. & 5 June 2019 & 0 & 444\\
            Jackal & A cloud storage solution. & 22 Oct. 2022 & 0 & 257\\
            Medibloc & A patient-centered health data ecosystem. & 26 Aug 2019 & 14,101 & 513\\
            Desmos & A framework to build social media platforms. & 10 Dec. 2019 & 3,202 & 758\\
            Dig& Tokenized real-estate. & 13 Dec. 2021 & 1,370 & 2\\\bottomrule
        \end{tabular}
    \end{table*}
}


==> Content/tmp.tex <==
\item[1] \url{https://github.com/Stride-Labs/stride/} v9.0.0
            \item[2] \url{https://github.com/osmosis-labs/osmosis} v15.1.0
            \item[3] \url{https://github.com/cosmos/gaia} v3.0.0
            \item[4] \url{https://github.com/axelarnetwork/axelar-core} v0.33.0
            \item[5] \url{https://github.com/crypto-org-chain/chain-main} v4.2.4
            \item[6] \url{https://github.com/fetchai/fetchd} v0.10.7
            \item[7] \url{https://github.com/regen-network/regen-ledger} v5.0.0
            \item[8] \url{https://github.com/JackalLabs/canine-chain} v1.2.0
            \item[9] \url{https://github.com/medibloc/panacea-core} v2.1.0
            \item[10] \url{https://github.com/desmos-labs/desmos} v5.0.0
            \item[11] \url{https://github.com/notional-labs/dig} v3.3.1
